Factual and Edit-Sensitive Graph-to-Sequence Generation via Graph-Aware Adaptive Noising

Fine-tuned autoregressive models for graph-to-sequence generation (G2S) often struggle with factual grounding and edit sensitivity. To tackle these issues, we propose a non-autoregressive diffusion framework that generates text by iterative refinement conditioned on an input graph, named as Diffusion Language Model for Graphs (DLM4G). By aligning graph components (entities/relations) with their corresponding sequence tokens, DLM4G employs an adaptive noising strategy. The proposed strategy uses per-token denoising error as a signal to adaptively modulate noise on entity and relation tokens, improving preservation of graph structure and enabling localized updates under graph edits. Evaluated on three datasets, DLM4G consistently outperforms competitive G2S diffusion baselines trained on identical splits across both surface-form and embedding-based metrics. DLM4G further exceeds fine-tuned autoregressive baselines up to 12x larger (e.g., T5-Large) and is competitive with zero-shot LLM transfer baselines up to 127x larger. Relative to the strongest fine-tuned PLM baseline, DLM4G improves factual grounding (FGT@0.5) by +5.16% and edit sensitivity (ESR) by +7.9%; compared to the best diffusion baseline, it yields gains of +3.75% in FGT@0.5 and +23.6% in ESR. We additionally demonstrate applicability beyond textual graphs through experiments on molecule captioning, indicating the method's generality for scientific G2S generation.

==> Background_and_Related_Work.tex <==
\section{Background and Preliminaries}\label{sec:background}

% We review graph-to-sequence (G2S) generation and briefly summarize Denoising Diffusion Probabilistic Models (DDPMs), which we later adapt for graph-conditioned sequence generation; additional details is in Appendix~\ref{App:related}.




\subsection{Related Work}
\textbf{Graph-to-Sequence Learning.}
G2S has progressed from (i) template-based systems \cite{kasner-dusek-2022-neural, vejvar-fujimoto-2023-aspiro}, to (ii) neural encoder--decoders with learned graph representations \cite{ribeiro-etal-2020-modeling, schmitt2021}, and (iii) fine-tuned transformer-based models that achieve competitive performance on standard surface metrics (BLEU, chrF++, METEOR) even without explicit graph-specific inductive biases \cite{ribeiro-etal-2021-investigating, NIPS2017_3f5ee243}.
This evolution motivates revisiting whether standard-metric performance also implies faithful realization of the input graph.

\textbf{PLMs for Graph Verbalization.}
A common strategy is to serialize the input graph (e.g., a KG) into a sequence of relational triples using special markers such as \texttt{[HEAD]}, \texttt{[REL]}, \texttt{[TAIL]}, and \texttt{[SEP]} (see Section~\ref{Graph_representation}). This enables direct use of standard encoder--decoder Transformers, but it gives up strict permutation invariance, a trade-off we revisit in Limitations~\ref{sec:limitations}. Recent work also highlights challenges in (i) aligning graph elements to text and (ii) representing multi-level semantics across nodes, edges, and subgraphs \cite{zhu2025llmgnngraphvocabulary}. While PLM-based approaches can be fluent, they remain constrained by left-to-right decoding, which can amplify early commitments and make local input edits propagate unpredictably \cite{ gong2023diffuseqsequencesequencetext}.

\textbf{Diffusion Models for Conditional Generation.}
Diffusion models provide a non-autoregressive alternative that generates by iterative refinement. In text, early approaches such as Diffusion-LM \cite{li2022diffusionlmimprovescontrollabletext} and Analog Bits \cite{chen2023analog} explored controllable generation in continuous representations, while DIFFUSEQ \cite{gong2023diffuseqsequencesequencetext} introduced sequence-to-sequence conditioning for diffusion language models. \texttt{DLM4G} builds on this line by conditioning explicitly on a serialized knowledge graph and introducing graph-aware adaptive noising to better preserve and recover graph-aligned components.

\textbf{Molecule Captioning.}
Graph-to-text generation is also central in scientific domains such as molecule and protein captioning \cite{edwards-etal-2022-translation, LIU2024108073, kim2025grapht5unifiedmoleculargraphlanguage, fei2025prot2textv2proteinfunctionprediction}. We include molecule captioning as an additional evaluation setting for graph-conditioned diffusion-based G2S. Table~\ref{tab:comparison} compares prior paradigms with \texttt{DLM4G}.

\subsection{Preliminaries: Denoising Diffusion Models}

DDPMs learn a data distribution over continuous variables, optionally conditioned on context $\mathbf{c}$, denoted $p(\mathbf{z}_0 \mid \mathbf{c})$. They consist of a fixed forward diffusion process and a learned reverse denoising process.

\textbf{Forward process.}
A standard DDPM forward process corrupts clean data $\mathbf{z}_0$ through a Markov chain with noise-schedule coefficients $\{\alpha_t\}_{t=1}^T$ controlling signal decay. This yields a closed-form for sampling a noised state $\mathbf{z}_t$ at any timestep $t$: $\mathbf{z}_t = \sqrt{\bar{\alpha}_t}\,\mathbf{z}_0 + \sqrt{1 - \bar{\alpha}_t}\,\boldsymbol{\epsilon},$
$\text{with} \quad
    \bar{\alpha}_t = \prod_{s=1}^t \alpha_s
    \ \text{and} \
    \boldsymbol{\epsilon}\sim\mathcal{N}(\mathbf 0,\mathbf I)$. Standard diffusion models typically use a fixed, data-agnostic (isotropic) schedule.

\textbf{Reverse process with conditional denoising.}
The reverse process learns to recover the clean data $\mathbf{z}_0$ from pure noise $\mathbf{z}_T \sim \mathcal{N}(\mathbf 0,\mathbf I)$. Let $q(\mathbf{z}_{1:T}\mid \mathbf{z}_0)$ denote the forward diffusion distribution. The learned reverse model defines a Markov chain $p_\theta(\mathbf{z}_{0:T}\mid \mathbf{c})$ where each transition
$p_\theta(\mathbf{z}_{t-1} \mid \mathbf{z}_t, \mathbf{c})$ is Gaussian with parameters predicted by a neural network $\mathcal{M}_\theta(\mathbf{z}_t,t,\mathbf{c})$ (e.g., via a parameterization of $\boldsymbol{\mu}_\theta$ and $\boldsymbol{\Sigma}_\theta$).
The parameters $\theta$ are optimized by maximizing a variational lower bound (VLB) on the conditional log-likelihood:
\vspace{-3mm}
\begin{equation}
\label{eq:vlb}
\resizebox{\columnwidth}{!}{$
\begin{aligned}
\mathcal{L}_{\text{vlb}}
= \mathbb{E}_{q}\Big[
\underbrace{-\log p_\theta(\mathbf{z}_0 \mid \mathbf{z}_1, \mathbf{c})}_{\text{Reconstruction }(L_0)}
 + \sum_{t=2}^{T}
\underbrace{
D_{\mathrm{KL}}\!\Big(
q(\mathbf{z}_{t-1} \mid \mathbf{z}_t, \mathbf{z}_0)\ \|\ 
p_\theta(\mathbf{z}_{t-1} \mid \mathbf{z}_t, \mathbf{c})
\Big)
}_{\text{Denoising matching }(L_{t-1})}
\\
+ \underbrace{
D_{\mathrm{KL}}\!\Big(
q(\mathbf{z}_T \mid \mathbf{z}_0)\ \|\ p(\mathbf{z}_T)
\Big)
}_{\text{Prior matching }(L_T)}
\Big].
\end{aligned}
$}
\end{equation}


While tractable, direct optimization of the full VLB is often unstable~\citep{li2022diffusionlmimprovescontrollabletext}; in later sections we show the modified objective with graph-aware, component-wise noising.
\begin{figure*}[t!]
    \centering
    \includegraphics[width=0.8\linewidth, height = 4cm]{images/framework.png}
    \caption{\texttt{DLM4G} framework:
(A) Graph-Sequence alignment set \{$\mathcal{A}$\}, obtains the aligned tokens;
(B) The model is trained with a graph-aware noising schedule
(C) Trained \texttt{DLM4G} samples output sequence conditioned on graph.}
\vspace{-5mm}
    \label{dlm4g}
\end{figure*}

